Cross-region Model Training with Communication-Computation Overlapping and Delay Compensation

Training large language models (LLMs) requires massive computational resources, often necessitating the aggregation of geographically distributed data centers (\ie, cross-region training). However, the high communication latency in wide-area networks severely degrades the efficiency of traditional distributed training. While methods like DiLoCo reduce communication frequency, they suffer from blocking synchronization. Streaming DiLoCo alleviates this issue via communication-computation overlapping but introduces update staleness and model inconsistency due to delayed global updates and partial synchronization. These factors impair convergence, especially when aggressive overlap is needed to mask high latency. We propose CoCoDC, a novel distributed training framework with communication-computation overlapping and delay compensation, to explicitly tackle these challenges. Within the CoCoDC framework, we specifically develop a novel Delay Compensation strategy based on Taylor expansion to effectively mitigate the staleness and an Adaptive Transmission strategy that dynamically schedules model fragment synchronization to optimize bandwidth usage and accelerate convergence. Extensive experiments highlight the superior performance of CoCoDC over both DiLoCo and Streaming DiLoCo regarding final accuracy and training speed. Specifically, CoCoDC reduces the training steps needed to reach a comparable perplexity by up to 21.0% compared to Streaming DiLoCo. Our work provides an effective solution for scalable and efficient cross-region LLM training.

==> contents/5.algo.tex <==

**3. The DC-DiLoCo Algorithm**

The DC-DiLoCo algorithm integrates staleness compensation into the Streaming DiLoCo training loop. Let $t$ denote the global step counter (incremented after each gradient accumulation cycle). Each worker $m$ maintains its local model parameters $\theta_m^{(t)}$ and potentially internal optimizer states. The synchronization occurs in fragments based on a schedule. We define $H$ as the macro-synchronization interval (all fragments are synchronized once within $H$ steps), $P$ as the number of fragments, and $H_p = H/P$ as the average interval between synchronizing the same fragment $p$. The communication-computation overlap depth is $\tau$ steps. $\lambda$ is the delay compensation coefficient.

**3.1 Parameter Sharding**

The model parameters are divided into $P$ shards. In our current implementation, we employ a simple layer-based strided partitioning. For a model with $L_{total}$ layers, we group consecutive layers into shards, aiming for roughly equal parameter counts or layer counts per shard. For instance, with $P$ shards, shard $p$ might contain layers $p, p+P, p+2P, ...$. (The specific sharding strategy `get_layer_shards` details this). Each worker maintains a `shard_tracker` dictionary to manage the state for each shard $p$, including:
*   `param_refs_p`: References to the actual model parameters $\theta_{m,p}^{(t)}$ belonging to shard $p$.
*   `params_p`: The globally agreed-upon parameters for shard $p$ from its last synchronization, $\theta_{global, p}^{(t_{rec}-H_p)}$. This serves as the base for the outer gradient calculation.
*   `staged_params_p`: A snapshot of the worker's local parameters for shard $p$ taken at the time its pseudo-gradient calculation started, $\theta_{m, p}^{(t_{rec})}$. Here $t_{rec}$ is the step when the *previous* synchronization cycle for shard $p$ was initiated (i.e., when the pseudo-gradient send started $\tau$ steps ago).
*   `outer_optimizer_p`: An optional separate optimizer (e.g., SGD Nesterov) acting on `params_p`.

**3.2 Training Loop and Synchronization (`sync_model`)**

The training proceeds similarly to standard distributed training with gradient accumulation. The key difference lies in the periodic `sync_model` calls integrated within the loop.

**Algorithm 1: DC-DiLoCo Worker Training Step (Conceptual)**

1: **Input:** Current global step $t$, local model $\theta_m^{(t)}$, local data batch $B_t$, local optimizer $Opt_{inner}$, shard tracker `tracker`
2: **Output:** Updated local model $\theta_m^{(t+1)}$
3.  // --- Inner Optimization Loop ---
4: Compute local gradient $\nabla L(B_t, \theta_m^{(t)})$
5: Accumulate gradient
6: **if** $(t+1)$ % `gradient_accumulation_steps` == 0 **then**
7:  Apply $Opt_{inner}$ step to get $\theta_m^{(t+1)}$ (includes gradient clipping, scheduler step)
8:  Zero gradients
9: // --- Synchronization Check & Execution ---
10: **for** each shard $p \in \{1, ..., P\}$ **do**
11:  **if** $t+1 == \text{tracker}_p[\text{'next_receive_step'}]$ **then** // Time to apply delayed update for shard p
12:   $\text{comm_time} \leftarrow \text{SyncModel}(\theta_m^{(t+1)}, \text{tracker}_p, p, \lambda, \tau, H_p)$
13:   // $\theta_{m,p}^{(t+1)}$ is potentially updated inside SyncModel
14:  **end if**
15:  **if** $(t+1) \% H_p == \text{sync_offset}_p$ **then** // Time to start sync cycle for shard p
16:   $\text{tracker}_p[\text{'staged_params'}] \leftarrow \text{clone}(\theta_{m,p}^{(t+1)})$ // Record current local state
17:   $\text{tracker}_p[\text{'sent_at_step'}] \leftarrow t+1$
18:   $\text{tracker}_p[\text{'next_receive_step'}] \leftarrow t+1+\tau$
19:   // Initiate non-blocking AllReduce for pseudo-gradient (logic inside SyncModel, called at receive time)
20:  **end if**
21: **end for**
22: **end if**


**Algorithm 2: `SyncModel` Function (Shard `p`)**

1: **Input:** Current model $\theta_m$, shard tracker `cur_shard`, shard index $p$, compensation factor $\lambda$, delay $\tau$, sync interval $H_p$
2: **Output:** Potentially updated parameters $\theta_{m,p}$
3: `param_refs_p` $\leftarrow$ `cur_shard`["param_refs"] // Refs to current model params for shard p
4: `params_p` $\leftarrow$ `cur_shard`["params"] // Global state from $t_{rec}-H_p$
5: `staged_params_p` $\leftarrow$ `cur_shard`["staged_params"] // Local state from $t_{rec}$ (recorded $\tau$ steps ago)

6: // --- 1. Calculate Outer Pseudo-Gradient Δm,p ---
7: `pseudo_grads_m,p` $\leftarrow$ `params_p` - `staged_params_p`

8: // --- 2. Communicate and Average: Δp = Avg(Δm,p) ---
9: `flat_pseudo_grads` $\leftarrow$ flatten(`pseudo_grads_m,p`)
10: `RingAllReduce`(`flat_pseudo_grads`, op=SUM) // Non-blocking initiated earlier, conceptually completed here
11: `flat_pseudo_grads` $\leftarrow$ `flat_pseudo_grads` / $M$
12: `avg_delta_p` $\leftarrow$ unflatten(`flat_pseudo_grads`, structure_like=`params_p`)

13: // --- 3. Apply Outer Optimization ---
14: **if** `cur_shard`["outer_optimizer"] **then**
15:  Apply `avg_delta_p` as gradient to `params_p` using `outer_optimizer_p`
16: **else** // Simple averaging (SGD, lr=1.0)
17:  `params_p` $\leftarrow$ `params_p` - `avg_delta_p`
18: **end if**
19: // `params_p` now holds the delayed global state $\theta_{global\_delayed, p}^{(t_{now})}$

20: // --- 4. Staleness Compensation (DC-S3GD inspired) ---
21: `current_local_params_p` $\leftarrow$ `param_refs_p` // $\theta_{m, p}^{(t_{now})}$
22: // Calculate local average velocity over last τ steps
23: `g_1` $\leftarrow$ (`staged_params_p` - `current_local_params_p`) / $\tau$
24: // Calculate divergence D between delayed global and past local state
25: `receive_interval` $\leftarrow$ $H_p$ // Approximation
26: `D` $\leftarrow$ (`params_p` - `staged_params_p`) / `receive_interval`
27: // Calculate compensated velocity
28: `g_1_corrected` $\leftarrow$ `g_1` + $\lambda \times$ (`g_1` $\odot$ `g_1`) $\odot$ `D`

29: // --- 5. Apply Compensated Update (Overwrite local state) ---
30: `w_corrected_p` $\leftarrow$ `params_p` + `g_1_corrected` $\times \tau$ // Predict current global state
31: **atomic** update `param_refs_p`.data $\leftarrow$ `w_corrected_p`.data

32: // --- 6. Cleanup (Optional state reset can happen here or before next send) ---
33: `cur_shard`["staged_params"] $\leftarrow$ None

**3.3 Theoretical Considerations (Preliminary)**

Providing a rigorous convergence analysis for DC-DiLoCo, which combines infrequent synchronization, streaming, overlap, non-linear inner/outer optimizers (AdamW/SGD-Nesterov), and the proposed compensation mechanism, is highly challenging and beyond the scope of this initial work.

However, we can offer some intuition. The convergence of DiLoCo relies on the assumption that the averaged pseudo-gradient $\bar{\Delta}_p$ provides a reasonable descent direction for the outer optimizer, despite being calculated based on local states. Streaming introduces inconsistency, while overlap introduces staleness ($\tau$ delay). Our compensation term aims to correct the update derived from the delayed global state ($\theta_{global\_delayed, p}^{(t_{now})}$) by incorporating the recent local trend (`g_1`) adjusted by the divergence (`D`) and a Hessian approximation (`g_1 \odot g_1`).

The effectiveness hinges on how well `g_1` captures the relevant local dynamics during the delay period and how accurately the term $\lambda (g_1 \odot g_1) \odot D$ corrects for the staleness. If the compensation is effective, it should bring the update closer to what would have happened with zero delay, potentially recovering some of the convergence speed lost due to staleness. The overwrite mechanism (Step 31 in Alg 2), however, deviates significantly from standard update rules and its theoretical impact requires careful study; it might lead to oscillations or loss of locally learned information if `w_corrected_p` is inaccurate. Future work should focus on bounding the error introduced by the compensation and the overwrite step within existing convergence frameworks for asynchronous or delayed optimization methods like those for ASGD or DiLoCo, potentially under simplifying assumptions (e.g., convex objectives, simpler optimizers).


==> contents/6.works.tex <==
% \subsection{Personalized Federated Learning} 
Personalized federated learning has gained increasing attention in recent years due to the prevalence of non-IID data in realistic environments\cite{tanPersonalized2022}.
Current researchers have made efforts to solve the statistical heterogeneity in PFL from different perspectives\cite{duanSelfBalancing2021,zhaoFederated2022,jiangImproving2023,nicholFirstOrder2018,arivazhaganFederated2019,liFedMD2019,corinziaVariational2021,huangPersonalized2021,shohamOvercoming2019,sattlerClustered2021,ghoshEfficient2022,yangPersonalized2023}.
For instance, cluster-based CFL by Sattler \etal \cite{sattlerClustered2021} and IFCA by Ghosh \etal \cite{ghoshEfficient2022} group clients into clusters based on specific metrics that estimate the similarity between clients.
However, these methods incur high computation and communication overhead due to the need to identify cluster structures or maintain multiple models.
In addition, methods like FedPer by Arivazhagan \etal \cite{arivazhaganFederated2019} split a model into a globally shared feature extraction part and a personalized local classification part. 
Clients combine these parts into a personalized model for local training, uploading only the feature extraction part for aggregation. 
Although FedPer directly generates personalized models and avoids the expensive computation overhead, it struggles to determine the optimal split layer and suffers from poor performance for unseen clients who do not participate in training.
To reduce computation overheads and generate personalized models for unseen clients, federated meta-learning is proposed and it incorporates meta-learning with FL and allows clients to generate personalized models on their own\cite{fallahPersonalized2020, jiangImproving2023,nicholFirstOrder2018,yueEfficient2021, renTinyReptile2023}.
Most FML approaches are based on MAML, a gradient-based meta-learning algorithm developed by Finn \etal \cite{finnModelAgnostic2017} and a first-order version of MAML termed Reptile proposed by Nichol \etal \cite{nicholFirstOrder2018}.
Fallah \etal \cite{fallahPersonalized2020} propose a pioneering FML algorithm Per-FedAvg to enhance learning on few-shot classification tasks.
Yue \etal \cite{yueEfficient2021} propose NUFM to conduct FML over multi-access wireless networks, and Ren \etal \cite{renTinyReptile2023} propose TinyReptile to conduct meta-learning on extremely resource-constraint devices such as micro control units.
However, these methods either do not explicitly accommodate system heterogeneity or do not optimize the inner-update frequency and meta-update frequency to achieve a trade-off between training efficiency and model performance.

Apart from the optimization of the training procedure, the evaluation metric for clients' dataset quality is also important for performance optimization in FML. 
Studies in meta-learning have explored enhancing meta-model performance by adjusting learning rates\cite{chenRobust2022} or actively selecting learning tasks\cite{yaoMetalearning2021, chenNearOptimal2022}.
For example, Chen \etal \cite{chenNearOptimal2022} use entropy changes before and after excluding a task to assess the task's importance, which is also known as informativeness.
However, the direct access to raw data limits its application in FL.
In information theory, Xu \etal \cite{xuTheory2020} propose usable information and extend conventional Shannon entropy under computational constraints, and Ethayarajh \etal \cite{ethayarajhUnderstanding2022} further develop it to estimate sample-level information extractable by ML models.
Rahman \etal \cite{rahmanFedPseudo2023} propose FedPseudo which employs UI to measure the effectiveness of augmenting Survival Analysis datasets by generating pseudo values.
However, UI is not used to guide the training phase in FedPseudo, which is different from our approach.

% % Meta-learning \cite{jiangImproving2023,nicholFirstOrder2018}, as mentioned in Section \ref{sec:intro}, aims at training a good initialization point for personalized models. 
% % However, current approaches often do not consider dataset intrinsics and system heterogeneity, leading to inefficient model training.
% % Data-based PFL methods primarily focus on mitigating data distribution disparities among clients.
% % Techniques such as data augmentation through up-sampling or down-sampling \cite{duanSelfBalancing2021,zhaoFederated2022} have been proposed to balance data distributions.
% % However, these operations can be unstable, potentially introducing bias or overfitting. 
% % For instance, aggressive oversampling of minority classes may lead to overfitting of those classes, while undersampling may result in loss of important information.
% % Client selection methods\cite{liFedSAE2021,yangFederated2020} attempt to identify clients with similar data distributions. 
% % While these methods can improve model performance, frequent selection of certain clients can lead to unfair resource allocation and potential privacy risks for frequently chosen clients, while less chosen clients may suffer from reduced model performance due to limited participation.
% Data-based PFL methods focus on mitigating data distribution disparities among clients. 
% Techniques such as data augmentation\cite{duanSelfBalancing2021,zhaoFederated2022} aim to balance data distributions through oversampling or undersampling, but risk overfitting or information loss. 
% Client selection methods\cite{liFedSAE2021,yangFederated2020} identify clients with similar data distributions, potentially improving model performance but raising concerns about resource allocation fairness and privacy.

% % Model-based techniques encompass various strategies to personalize models.
% % Meta-learning \cite{jiangImproving2023,nicholFirstOrder2018}, as mentioned in Section \ref{sec:intro}, aims at training a good initialization point for personalized models. 
% % However, current approaches often do not consider dataset intrinsics and system heterogeneity, leading to inefficient model training.
% % Transfer learning\cite{yang2020fedsteg,chen2020fedhealth} can also generate personalized models by fine-tuning a model pre-trained on data within a related but different source domain. However, these methods may struggle with negative transfer where source and target domains are dissimilar and inadvertently leak information about the source domain.
% Model-based techniques include meta-learning and transfer learning. 
% Current meta-learning\cite{jiangImproving2023,nicholFirstOrder2018}, as mentioned in Section \ref{sec:intro}, aims to train a good initialization point for personalized models but often overlooks dataset intrinsics and system heterogeneity. 
% Transfer learning\cite{yang2020fedsteg,chen2020fedhealth} can generate personalized models through fine-tuning but may struggle with negative transfer and inadvertent information leakage.

% % Architecture-based methods focus on learning personalized models through structural modifications. 
% % Splitting models into personalized layers can generate localized feature extraction layers\cite{buiFederated2019} or classification layers\cite{arivazhaganFederated2019} and adapt to client-specific data.
% % While such methods demonstrate strong interpretability, determining the optimal model split point remains challenging.
% % Knowledge distillation enables knowledge sharing between heterogeneous model structures\cite{liFedMD2019,linEnsemble2021}, but transmitting soft logits can expose the system to security vulnerabilities, such as model inversion attacks.
% Architecture-based methods learn personalized models through structural modifications. 
% Splitting models into personalized layers\cite{buiFederated2019,arivazhaganFederated2019} such as individual feature extraction modules and classification modules can adapt to client-specific data, but faces challenges in determining optimal model split points. 
% Knowledge distillation\cite{liFedMD2019,linEnsemble2021} enables knowledge sharing between heterogeneous model structures but may expose the system to security vulnerabilities since soft-logit transmissions are required.

% % Similarity-based approaches aim to model relationships between clients. 
% % For example, multi-task learning treats clients as different tasks and seeks latent relationships between heterogeneous data\cite{corinziaVariational2021,huangPersonalized2021,shohamOvercoming2019}. 
% % While effective, MTL can be computationally intensive due to the need for simultaneously optimizing multiple loss functions and managing complex data dependencies. 
% % Clustering clients into groups with high intra-cluster similarity offers a direct solution to the one-size-fits-all problem. 
% % Methods such as bi-partitioning clients based on gradient cosine similarity\cite{sattlerClustered2021} and selecting clients with the lowest local loss on different global models\cite{ghoshEfficient2022} exemplify this approach. 
% % However, these methods are often computationally and storage intensive due to the need for similarity computation or maintaining cluster centers, making them less practical for real-time, large-scale FL applications.

% % We believe PFL is an important underscored area for future FL research, as modern edge devices are generating unprecedented amounts of data, and becoming more powerful and capable of running complex models.


% Similarity-based approaches model relationships between clients. 
% Multi-task learning\cite{corinziaVariational2021,huangPersonalized2021,shohamOvercoming2019} treats clients as different tasks. 
% But simultaneously optimizing multiple loss functions can be computationally intensive. 
% Clustering clients with high intra-cluster similarity\cite{sattlerClustered2021,ghoshEfficient2022,yangPersonalized2023} offers a direct solution to the one-size-fits-all problem but often requires significant computational and storage resources.

% \subsection{Information Theory in FL} 
% While PFL approaches show promise, they often lack an understanding of client datasets' informativeness. 
% This gap motivates the exploration of information theory in FL contexts,  which can provide valuable insights into dataset characteristics and guide personalization strategies.

% Shannon entropy\cite{shannonMathematical1948} has long been a well-known metric for measuring information content in messages or other data. 
% However, it falls short in high-dimensional data contexts, making it unsuitable for measuring complex real-world data such as images. 
% To address this limitation, \V-entropy and \V-usable information \V-usable information are proposed as more general and effective measures for high-dimensional data \cite{xuTheory2020}. 
% Generally speaking, \V-usable information uses machine learning models' performance gap on a normal dataset and the modified version of the dataset without side information to show whether the data are informative or not, which we will detail in the following section.
% These metrics extend conventional Shannon entropy under computational constraints, making them suitable for machine learning data estimation.

% The applicability of these information-theoretic measures has been demonstrated in various ML contexts. 
% In natural language processing, studies \cite{ethayarajhUnderstanding2022} leveraged \V-entropy to estimate the information content of multiple datasets, correlating with the performance of models like BERT \cite{devlinBERT2019} and GPT-2 \cite{radfordLanguage2019}. 
% Research \cite{cuiLearning2023} effectively used large-scale pre-trained models and \V-entropy to train downstream models and prevent overfitting. 
% Study \cite{rahmanFedPseudo2023} employed \V-usable information to measure the effectiveness of augmenting Survival Analysis datasets by generating pseudo values where real values are unavailable in FL.
% However, the \V-usable information is only used during the centralized evaluation phase.
% There are still some challenges to be addressed, such as how we can further reduce the overhead of calculating UI and how to obtain a uniform method of selecting or deciding training parameters to improve the precision of UI estimation.
% Another possible research direction is how to utilize UI into non-classification tasks.

% Our work expands the application of \V-inf to estimate the information content of image classification datasets in a distributed environment. 
% We integrate this approach with meta-learning techniques and consider system heterogeneity to address the limitations of current PFL methods. 
% By incorporating information-theoretic measures into PFL, we aim to provide a more nuanced understanding of client datasets, enabling more effective personalization strategies. 


==> contents/backup/1.intro-backup0423.tex <==
The landscape of artificial intelligence (AI) has been dramatically reshaped by the advent of large language models (LLMs) \cite{minaeelarge2025}. 
These models, boasting billions or even trillions of parameters, have demonstrated remarkable capabilities across a wide spectrum of natural language tasks. 
However, training such colossal models demands unprecedented computational resources, often requiring thousands of high-end accelerators (like GPUs or TPUs) running for weeks or months. 
While scaling up resources within a single data center cluster has been the default approach, it is increasingly facing bottlenecks related to power delivery, cooling infrastructure, and sheer physical space limitations. 

To harness geographically dispersed computational power, training LLMs across multiple data centers (DCs) over wide-area networks (WANs) emerges as a compelling necessity. 
By aggregating idle or underutilized resources from different locations, organizations can potentially shorten the lengthy training cycles, reduce the substantial costs associated with dedicated clusters, and accelerate the pace of model development and iteration. 
This distributed paradigm is particularly relevant in cross-silo or cross-region scenarios involving federated learning (FL) \cite{mcmahancommunicationefficient2023} across different enterprise branches or collaborative research efforts spanning multiple institutions, where data locality and privacy concerns might also preclude centralizing all data for analysis. 
However, the substantial communication latency in WANs critically hinders traditional distributed training, particularly data parallelism (DP). 
DP’s reliance on synchronous stochastic gradient descent (SSGD) \cite{chenrevisiting2017} mandates global gradient synchronization before each training step, forcing workers to idle and severely underutilizing resources. 
This inefficiency worsens with LLMs, as their massive parameter sizes drastically amplify communication overhead, leading to prolonged training delays.

To mitigate the high communication costs associated with cross-silo environments, methods focusing on infrequent synchronization have been proposed. 
A prominent example is DiLoCo\cite{douillarddiloco2024} (referred to as Distributed Low-Communication), which allows DCs acting as workers to perform multiple local computation steps (denoted by $H$) before synchronizing their local updates (\ie, pseudo-gradients) globally in an All-Reduce operation. 
While DiLoCo effectively reduces communication frequency, it suffers from two primary limitations. 
% Firstly, \rednote{the global synchronization step remains blocked:} %这里最好换个表述，使得和后面能够衔接成一个完整句子。
% all workers must pause their local computations and wait for \rednote{the slowest worker} %感觉这里可以先不说系统异构的问题，先说明传、算串行对资源的利用率影响的问题。
% to complete communication phases before proceeding. 
Firstly, the global synchronization step incurs a bottleneck, as all workers must suspend local processing until the communication phase completes.
% The serialized exectuion of computation and communication always leads to significant resource wastage, thereby diminishing end-to-end wall-clock time efficiency. 
This serialized execution of computation and communication inherently leads to severe resource underutilization, as computational resources remain idle during communication phases, and network bandwidth goes unused during computation phases, diminishing end-to-end wall-clock time efficiency.
Secondly, despite the reduced frequency, each synchronization event in DiLoCo requires all workers to simultaneously transmit their entire model's pseudo-gradients. %这里是不是应该强调下所有worker同时发送的问题？ 
This results in prohibitive peak bandwidth demands for environments constrained by low bandwidth or expensive inter-DC links.

Aiming to overcome the limitations of DiLoCo, Streaming DiLoCo \cite{douillardstreaming2025}, an advanced variant of DiLoCo, introduces optimizations through two key mechanisms: 
(a) Streaming Synchronization: The model parameters and their corresponding pseudo-gradients are partitioned into smaller fragments alongside the depth direction. 
These fragments are then synchronized sequentially according to a predefined schedule (\eg, evenly distributed across the $H$ local training steps), %这里具体明确一下是什么策略
effectively smoothing out the peak bandwidth requirement compared to synchronizing the entire model simultaneously. 
(b) Communication-Computation Overlapping: 
Workers can perform local computations on subsequent data batches while exchanging pseudo-gradient fragments from previous steps. 
% This overlap, typically parameterized by $\tau$ steps, \rednote{aims to hide the communication latency}, %这里表述不够充分
% thereby improving computational resource utilization and accelerating the overall training process.
This overlap, typically parameterized by $\tau$ steps, aims to hide communication latency by allowing workers to train concurrently with data transfer, thereby improving computational resource utilization and accelerating the overall training process.

However, these optimization mechanisms in Streaming DiLoCo introduce two new critical challenges: \textbf{staleness} and \textbf{inconsistency}. 
Staleness arises from the temporal delay: when a worker receives and applies a global pseudo-gradient update for a particular model fragment, the pseudo-gradient was computed based on the global model state from $\tau$ steps prior.
On the other hand, inconsistency stems from the partial nature of the updates inherent in streaming. 
At any given time, only the specific model fragment being synchronized incorporates the global information, while the remaining fragments retain their purely local state derived from the worker's independent computations. 
This creates an internal inconsistency across different parts of the model within a single worker. 
% \rednote{Both staleness and inconsistency, especially when the overlap depth $\tau$ or the local computation period $H$ is large, can lead to suboptimal parameter updates, potentially hindering convergence speed and degrading the final model performance.} %这里关于staleness和inconsistency对于训练的影响分析不够深刻。
In general, both staleness and inconsistency represent deviations from the ideal synchronous update process. 
Staleness introduces errors due to outdated gradient information, while inconsistency creates unaligned model states within a worker. 
Furthermore, when the overlap depth $\tau$ or the local step $H$ gets large, these deviations can accumulate, resulting in suboptimal parameter updates that hinder convergence speed and degrade final model performance.

To address the above issues in cross-silo LLM training, we propose a novel distributed training framework with communication-computation overlapping and delay compensation, termed \method.
\method introduces explicit mechanisms to mitigate the detrimental effects of staleness and inconsistency.
Specifically, we leverage Taylor expansion to approximate the ``ideal'' global pseudo-gradient information corresponding to the worker's current state, thereby compensating for the delay introduced by the overlap depth $\tau$ 
before applying the received update. 
Moreover, recognizing that not all model parameters contribute equally to convergence at all times, we design an adaptive model transmission algorithm. 
This algorithm allows for more strategic utilization of the available bandwidth by transmitting important or rapidly changing fragments
% model blocks 
multiple times within a local computation period $H$, ensuring critical updates are propagated more effectively, rather than rigidly adhering to a fixed transmission schedule.
In summary, the main contributions of this paper are: 
% 以下按照这三个方面进行组织：
% 1、针对DiLoCo里传算串行所导致的计算和通信资源利用不充分的问题，以及streaming DiLoCo里steleness和inconsistency所导致的xxx问题，我们提出了一个新的cross-silo LLM training framework来通过delay compensation消除xxx的影响。
% 2、进一步对框架做个说明，并说明我们通过什么算法或策略来消除staleness和inconsistency的负面影响。
% 3、实验表明，我们相比于DiLoCo和Streaming DiLoCo的性能提升情况。

\begin{enumerate}

\item We identify critical limitations in existing cross-silo methods: DiLoCo's serial execution leads to resource underutilization, while Streaming DiLoCo's overlap introduces staleness and inconsistency that can degrade convergence speed and final model performance. 
To address these, we propose \textbf{\method}, a novel distributed training framework specifically designed for efficient and robust cross-silo LLM training.

\item \method employs a Taylor expansion-based delay compensation mechanism to mitigate gradient staleness from communication overlap. 
Furthermore, it utilizes an adaptive block transmission strategy to optimize bandwidth and prioritize impactful parameter updates by transmitting them multiple times within the local computation period, 
enhancing overall update quality and mitigating inconsistency effects.

\item Our extensive experiments validate that \method significantly reduces wall-clock training time compared to DiLoCo and DP by effectively overlapping communication and compensating for delay. 
Moreover, \method demonstrates superior convergence speed compared to Streaming DiLoCo, requiring up to 21.0\% fewer training steps to achieve comparable perplexity.
\end{enumerate}


==> contents/backup/2.framework-backup0423.tex <==
We consider the scenario of training an LLM collaboratively across $M$ geographically distributed DCs connected using a decentralized, peer-to-peer (P2P) architecture, denoted as workers $W = \{w_1, w_2, ..., w_M\}$. 
Each worker $w_m$ is assumed to possess substantial computational capabilities, typically comprising a local cluster of accelerators, and holds a local data partition $D_m$.
The data across these DCs can be non-identically distributed (non-IID), reflecting realistic federated or collaborative settings.
Within its local environment, $w_m$ can leverage standard intra-node parallelism techniques (\eg, \rednote{DP, TP, PP}). %给出全称
However, these internal strategies are orthogonal to the inter-site coordination protocol that is the focus of this work.

The primary obstacle in this cross-DC environment lies in the excessive communication overhead incurred by synchronizing distributed model updates over WANs, which is typically characterized by high latency $L$ and limited bandwidth $B$. 
Traditional synchronous methods like standard DP, require blocked gradient synchronization (\eg, via ring all-reduce) after every computational step.
This leads to severe underutilization of \rednote{compute resources} and excessively long training times. 

To address this, DiLoCo reduces communication frequency by having each worker perform $H$ local training steps before engaging in a global synchronization.
Instead of gradients, workers synchronize their accumulated updates or pseudo-gradients, defined as the difference between their current local model $\theta^m_{t}$ and the globally agreed-upon model state from the previous synchronization round $\theta^g_{t-H}$. 
While effective in reducing the number of synchronization sessions, DiLoCo's global synchronization remains a blocking operation, forcing all workers to wait for the all-reduce. 
Furthermore, transmitting the entire model's pseudo-gradients, even infrequently, can still demand high peak bandwidth.

Streaming DiLoCo enhances efficiency by integrating two key ideas: model partitioning and communication-computation overlap. 
The model parameters $\theta$ are partitioned into $K$ disjoint shards $\{\theta_1, ..., \theta_K\}$. 
Instead of synchronizing the entire model every $H$ steps, synchronization happens shard-by-shard according to a schedule distributed across the $H$ local steps. 
Let $t_p$ be the local step at which worker $w_m$ initiates the synchronization process for shard $p$. 
The worker calculates the pseudo-gradient for this shard, $\Delta \theta^m_p = \theta^m_{p, t_p} - \theta^g_{p, t_p-H}$, where $\theta^g_{p, t_p-H}$ is the global state of shard $p$ from its last synchronization $H$ steps prior.
Then they start the Ring All-Reduce communication for $\Delta \theta^m_p$.
Crucially, the worker does \textit{not} wait for the communication to finish.
It immediately proceeds with local forward/backward passes on subsequent mini-batches.

After a certain duration, the communication for shard $p$ completes.
Since we allow computation to continue along with the communication session, currently workers would be at local steps $t_l = t_p + \tau$. 
The overlap duration $\tau$ represents the effective communication delay experienced by the worker for this shard synchronization and can vary depending on shard size $S_p$ and network conditions. 
At step $t_l$, an outer optimizer (\eg, SGD with Nesterov momentum) uses $\Delta \theta^g_p$ to update the shard's previous global state $\theta^g_{p, t_p-H}$ to compute the new target global state, denoted $\theta^{g}_{p, t_p}$:
\begin{align}
\label{eq:outer_grad_agg}
\Delta \theta^g_p &= \frac{1}{M} \sum_{m=1}^{M} (\theta^m_{p, t_p} - \theta^g_{p, t_p-H}) \\
\label{eq:outer_optim}
\theta^{g}_{p, t_p} &\leftarrow \text{OuterOptim}_p(\theta^g_{p, t_p-H}, \Delta \theta^g_p )
\end{align}
In Streaming DiLoCo, this newly computed target global state $\theta^{g}_{p, t_p}$ is typically blended with the worker's current local state for that shard $\theta^m_{p, t_l}$ using a mixing factor $\alpha$:
\begin{equation}
\label{eq:blending}
\theta^{m}_{p, t_l} \leftarrow (1-\alpha)\theta^{m}_{p, t_l} + \alpha \cdot \theta^{g}_{p, t_p}
\end{equation}
This blending step updates the worker's local model using the global information.
However, as discussed in the Section \ref{sec:introduction}, this overlap introduces staleness due to the $\tau$-step delay and inconsistency due to partial updates. 
The hyperparameter $\alpha$ also needs meticulous tuning for balancing between local and global updates.

Our proposed method, \method directly confronts these challenges by introducing delay compensation and adaptive update mechanisms into the streaming framework.
Instead of simply blending the stale global state, \method employs an explicit \textbf{Delay Compensation} mechanism. 
This mechanism leverages information available at the receiving step $t_l$, including the current local state $\theta^m_{p, t_l}$, the recorded local state from the time the synchronization started $\theta^m_{p, t_p}$, and the received averaged pseudo-gradient $\Delta \theta^g_p$. 
Using a Taylor expansion-based approach, it computes a \textit{corrected} update that aims to approximate the ideal global update corresponding to the current time $t_l$, effectively mitigating the negative impact of the $\tau$-step staleness. 
Furthermore, to combat inconsistency and improve bandwidth utilization beyond the rigid scheduling of Streaming DiLoCo, \method incorporates an \textbf{Adaptive Transmission Strategy}. 
This strategy estimates the maximum number of shards that could be transmitted during the computation time available within a synchronization cycle and tracks the magnitude of parameter changes since last synchronization. 
Instead of synchronizing each shard exactly once per $H$ steps, \method prioritizes transmitting additional copies of more critical shards within the available bandwidth and time window, aiming to propagate important updates faster and fill idle network capacity more effectively.

The core challenges in designing \method lie in formulating an effective and computationally feasible delay compensation calculation and developing a robust adaptive transmission strategy. 
We'll elaborate on the specific algorithms designed to address these challenges in Section \ref{sec:strategy}.

